Is this Snippet Written by ChatGPT? An Empirical Study with a CodeBERT-Based Classifier

Since its launch in November 2022, ChatGPT has gained popularity among users, especially programmers who use it as a tool to solve development problems. However, while offering a practical solution to programming problems, ChatGPT should be mainly used as a supporting tool (e.g., in software education) rather than as a replacement for the human being. Thus, detecting automatically generated source code by ChatGPT is necessary, and tools for identifying AI-generated content may need to be adapted to work effectively with source code. This paper presents an empirical study to investigate the feasibility of automated identification of AI-generated code snippets, and the factors that influence this ability. To this end, we propose a novel approach called GPTSniffer, which builds on top of CodeBERT to detect source code written by AI. The results show that GPTSniffer can accurately classify whether code is human-written or AI-generated, and outperforms two baselines, GPTZero and OpenAI Text Classifier. Also, the study shows how similar training data or a classification context with paired snippets helps to boost classification performances.

==> src/Study.tex <==

%In this section, w
We conduct a preliminary evaluation of our proposed approach using a real dataset. Section~\ref{sec:ResearchQuestions} presents two research questions, while Section~\ref{sec:Process} describes the evaluation process. Section \ref{sec:dataset} gives a detailed description of the dataset used for the evaluation, and the metrics are specified in Section~\ref{sec:metrics}. Section \ref{sec:results} discusses the results by answering the two research questions. %are discussed in .  %We measure.



\subsection{Research questions} \label{sec:ResearchQuestions}
%In this feasibility study, w
%We address t
The following research questions are considered:
%\begin{itemize}
%\item 

\noindent
$\rhd$~\rqfirst~To answer this question, we compute precision, recall, and F-measure, considering real migration data from \GH. Furthermore, we conduct experiments following the ten-fold cross-validation methodology on a well-founded dataset. %to achieve better results.

\noindent
$\rhd$~\rqsecond~Besides the recommended migration steps, we are interested in measuring the time of the overall process, including the graph building phase.
%\end{itemize}

\vspace{-.1cm}
\subsection{Overall process} \label{sec:Process}
\vspace{-.2cm}
%To answer the research questions, 
As depicted in Fig.~\ref{fig:eval}, we perform experiments using the ten-fold 
cross-validation methodology on a well-founded dataset coming from an existing 
work~\cite{kula_developers_2018}. Given a list of projects, we download the entire 
dataset using the Crawler component. Then, the dataset is split into testing and 
training projects, 10\% and 90\% of the entire set, respectively, by each round of the 
process. Given a single testing project, \emph{Commit Analyzer} is used to capture the 
actual upgrade path followed by the repository, as stated in Section \ref{sec:tracker}. 
Concerning the training process, we build a different migration graph and calculate 
every possible upgrade plan for each TPLs extracted from the original dataset. To aim 
for a reliable evaluation, we select the start and the end version of a certain TPL from 
the actual plan of a testing project. This pair is used to feed \emph{Plan Calculator} 
that retrieves the proposed plan. 
%As we are interested only in upgrades, we do not consider the downgrade cases, \ie in 
%which a certain library migrates to an older version.
In such a way, we can compute on the two paths the metrics to assess the overall 
performances, \ie precision, recall, and F-measure.


\begin{figure}[t!]
	\vspace{-.5cm}
	\centering
	\includegraphics[width=0.86\linewidth]{figs/Eval.pdf}
	\vspace{-.4cm}
	\caption{The evaluation process.}
	\vspace{-.6cm}
	\label{fig:eval}
\end{figure}

\vspace{-.1cm}
\subsection{Data gathering} \label{sec:dataset}
\vspace{-.2cm}
%Concerning the dataset, 
We exploit an existing dataset which has been curated by a recent 
study,\footnote{\url{https://github.com/raux/Impact-of-Security-Advisories-on-Library-Migrations}}
 available on \GH. The dataset consists of 10,952 \GH repositories. The 
rationale behind this choice is the quality of the repositories which were 
collected by applying different filters, \ie removing duplicates, including 
projects with at least one \emph{pom.xml}, and crawling only well-maintained 
and mature projects. This dataset has been used to collect statistical 
information about library usages and dependency update. %Considering the 
%imposed quality filter, we decide to employ this dataset in the evaluation of 
%our tool. 
%To aim for a reliable evaluation, we experiment using the ten-fold cross-validation technique: %splitting the dataset in testing and training projects for each round of validation.
The training set is used to create a migration graph to avoid any possible bias. For each round, we tested 420 projects, and 3,821 projects are used to build the graph. 

\vspace{-.1cm}
\subsection{Metrics} \label{sec:metrics}
\vspace{-.2cm}
%To assess the proposed approach, 
%We make use of precision, recall, F-measure to measure the quality of retrieved migration paths. In particular, 
Given a migration path retrieved by \tool, we compare it with the real migration path extracted from a testing project. There are the following definitions: \emph{TP} is true positive, corresponding to the case the recommended path matches with the actual path extracted from the testing projects; False positive (\emph{FP}) means that the recommended upgrade plan is not present in the testing projects; False negative (\emph{FN}) is the migration steps that should be present in the suggested plan but they are not. Considering such definitions, we compute \emph{Precision}, \emph{Recall}, and \emph{F-measure} (or F$_1$-score) as follows. %according to their standard formulas used in Information Retrieval:
%\begin{equation}
%P = \frac{ TP }{TP+ FP}
%\end{equation}
%
%\noindent
%\begin{equation} \label{eqn:Recall}
%R = \frac{ TP }{TP+FN}    
%\end{equation}



\begin{minipage}{0.48\linewidth}
	\begin{equation} \label{eqn:Precision}%\nonumber%
	P = \frac{ TP }{TP+ FP}
	\end{equation}
\end{minipage}% 
\begin{minipage}{0.48\linewidth}
	\begin{equation} \label{eqn:Recall}%\nonumber%
	R = \frac{ TP }{TP+FN}    
	\end{equation}
\end{minipage}%\par\vspace{\belowdisplayskip}


\begin{equation} \label{eqn:F-Measure}
F_1 = \frac{ 2 \times P \times R  }{P + R}    
\end{equation}

\vspace{-.1cm}
\subsection{Preliminary results} \label{sec:results}

We report and analyze the obtained results by answering the research questions introduced in Section~\ref{sec:ResearchQuestions} as follows.


\vspace{.1cm}
\noindent
$\rhd$~\rqfirst~We compute the above-mentioned metrics on seven different popular Java libraries according to the Maven Repository's statistics,\footnote{\url{https://mvnrepository.com/popular}} namely \emph{junit}, \emph{httpclient}, \emph{slf4-api}, \emph{log4j}, \emph{commons-io}, \emph{guava}, and \emph{commons-lang3}. Table \ref{tab:metrics} reports the average results for the cross-fold validation evaluation. %Overall, \tool reaches good performance by considering the average values of the metrics computed over the ten rounds of validation.

\vspace{-.4cm}
\begin{table}[h]
\centering
\caption{Precision, Recall, and F-Measure.}%Metrics' results
\vspace{-.3cm}
\begin{tabular}{|l | p{1.3cm} |  p{1.3cm} | p{1.3cm} |}
\hline
\textbf{Library} & \textbf{Precision} & \textbf{Recall} & \textbf{F-measure} \\ \hline
junit &  0.93 &	\textbf{0.98} &	0.95 \\ \hline
httpclient & 0.75 &	0.64 & 0.68  \\ \hline
slf4j-api & 0.98  &	0.83 &  0.88  \\ \hline
log4j & \textbf{1.00}	&  0.95	& 0.97  \\ \hline
commons-io & 0.97 & \textbf{0.98} &	\textbf{0.98}  \\ \hline
guava & 0.87	&  0.80  &	0.83 \\ \hline
commons-lang3 & 0.73  & 0.78 &	0.72 \\ \hline
\end{tabular}
\vspace{-.4cm}
\label{tab:metrics}
\end{table}

%In particular, we notice that 
\vspace{.2cm}
\tool achieves the maximum precision for \emph{log4j}, \ie P=1.0 in all the rounds. Concerning recall, a value of 0.98 is obtained for the \emph{junit} and \emph{commons-io} libraries. In contrast, the tool achieves the the worst recall values for \emph{httpclient}, \ie while the minimum precision value is observed for \emph{commons-lang3} library, 0.64 and 0.73 respectively. \tool gets the best performance concerning F-Measure for \emph{commons-io}, \ie the score is 0.98. Altogether, we see that there is substantial difference between the performance obtained by \tool for different libraries. We suppose that this happens due to the availability of training data. In particular, by carefully investigating the clients that invoke \emph{httpclient}, we see that there are few migration paths among them, and this should have a negative impact on the overall recommendation.

% records  of the entire dataset
%as the F-measure value overcomes the other libraries' results.
\vspace{.1cm}
\begin{tcolorbox}[boxrule=0.86pt,left=0.3em, right=0.3em,top=0.1em, bottom=0.05em]
	\small{\textbf{Answer to RQ$_1$.} \tool is capable of predicting the correct upgrade plan given a real-world migration dataset.}
\end{tcolorbox}

%: all the quality metrics reach high values considering real-world data
%Though this is a preliminary evaluation, 

\vspace{.1cm}
\noindent
$\rhd$~\rqsecond~%As the second research question,
We measured the average time required for running experiments using a mainstream laptop with the following information: i5-8250U, 1.60GHz Processor, 16GB RAM, Linux as operating system. The measured time performance is as follows: the querying phase takes just 0.11 seconds to finish; the testing phase is longer: 145.44 seconds; and the most time consuming phase is the creation of graph with 15,120 seconds, corresponding to 280 minutes. It is worth noting that the testing consists of the sub-operations that are performed in actual use, \ie opening CSV files, extracting the actual plan, and calculating the shortest path. Roughly speaking, this means that in one second we can get an update plan for three clients. This is acceptable, given that the laptop used for the measurement possesses an average computational capability. We suppose that with a more powerful computing platform, the time performance can substantially be improved.

%We see that.

%The testing phase for all considered TPLs requires around 145 seconds on average.


%Finally, we computed the time required for a complete round of
%creation of the graph, the testing phase, and . Figure~\ref{fig:time} summarizes such phases by measuring the required time in seconds.
%the following operations 
% involved in the whole process
%computer  All the time measurements have been computed on a 
%\begin{figure}[h]
%	\centering
%	\includegraphics[width=\linewidth]{figs/time.pdf}
%	\caption{Time required for each examined phase.}
%	\label{fig:time}
%\end{figure}

%As we can notice, graph creation is the most time consuming phase, it takes around 280 minutes to complete. Contrariwise, the recommendation of an upgrade path for a single TPL requires only 0,10 seconds on average. 



\begin{tcolorbox}[boxrule=0.86pt,left=0.3em, right=0.3em,top=0.1em, bottom=0.05em]
	\small{\textbf{Answer to RQ$_2$.} The creation of the migration graph is computationally expensive. However, it can be done offline, one time for the whole cycle. \tool is able to deliver a single upgrade plan in a reasonable time window, making it usable in the field.}
\end{tcolorbox}

%, and it can be done offline. 
%allows the usability of
%Concerning the recommendation phase, 

% it takes place at the beginning of the process
%Total number of repo & 10,000 & \textbf{Downloaded repo} & 9,517\\ 













